Data-rich astronomy: mining synoptic sky surveys

In the last decade a new generation of telescopes and sensors has allowed the production of a very large amount of data and astronomy has become, a data-rich science; this transition is often labeled as: "data revolution" and "data tsunami". The first locution puts emphasis on the expectations of the astronomers while the second stresses, instead, the dramatic problem arising from this large amount of data: which is no longer computable with traditional approaches to data storage, data reduction and data analysis. In a new, age new instruments are necessary, as it happened in the Bronze age when mankind left the old instruments made out of stone to adopt the new, better ones made with bronze. Everything changed, even the social structure. In a similar way, this new age of Astronomy calls for a new generation of tools and, for a new methodological approach to many problems, and for the acquisition of new skills. The attems to find a solution to this problems falls under the umbrella of a new discipline which originated by the intersection of astronomy, statistics and computer science: Astroinformatics, (Borne, 2009; Djorgovski et al., 2006).

==> FileTex/conclusionsscie.tex <==


\section{the animals}
\begin{equation}
{\begin{array}{*{20}c}
\overbrace{\bigodot\bigodot}\\
\bigvee
\end{array}} 
\end{equation}

\begin{equation}
\begin{array}{*{20}c}
   {\mathlarger{\bigcap\checkmark\bigcap}}  \\
   {\mathop {\bigodot\bigodot}\limits_{\nabla} }  \\
   {\sqcup\sqcup}  \\
\end{array}
\end{equation}



\begin{equation}
\begin{array}{*{20}c}
   {\mathlarger{\vartriangle\checkmark\vartriangle}}  \\
   {\mathop {\widehat{\bigodot}\widehat{\bigodot}} }  \\
     {\Theta}\\
\end{array}
\end{equation}


\begin{equation}
\tikz[baseline]{
\node[fill=red!10, circle,anchor=base] (puork)
{$\begin{array}{*{20}c}
   {\mathlarger{\vartriangle\checkmark\vartriangle}}  \\
   {\mathop {\widehat{\bigodot}\widehat{\bigodot}} }  \\
     {\Theta}\\
\end{array}$};
}
\end{equation}

\begin{equation*}
\vec{a}_p = \vec{a}_o+\frac{{}^bd^2}{dt^2}\vec{r} +
        \tikz[baseline]{
            \node[fill=blue!20,anchor=base] (t1)
            {$ 2\vec{\omega}_{ib}\times\frac{{}^bd}{dt}\vec{r}$};
        } +
        \tikz[baseline]{
            \node[fill=red!20, circle,anchor=base] (t2)
            {$\vec{\alpha}_{ib}\times\vec{r}$};
        } +
        \tikz[baseline]{
            \node[fill=green!20,anchor=base] (t3)
            {$\vec{\omega}_{ib}\times(\vec{\omega}_{ib}\times\vec{r})$};
        }
\end{equation*}


\clearpage \newpage 
\section{The Trolls}



\begin{verbatim}
                                ___________________________
                       /|  /|  |                          |
                       ||__||  |       Please don't       |
                      /   O O\__           feed           |
                     /          \       the trolls        |
                    /      \     \                        |
                   /   _    \     \ ---------------------- 
                  /    |\____\     \     ||                
                 /     | | | |\____/     ||                
                /       \|_|_|/   |    __||                
               /  /  \            |____| ||                
              /   |   | /|        |      --|               
              |   |   |//         |____  --|               
       * _    |  |_|_|_|          |     \-/                
    *-- _--\ _ \     //           |                        
      /  _     \\ _ //   |        /                        
    *  /   \_ /- | -     |       |                         
      *      ___ c_c_c_C/ \C_c_c_c__________
\end{verbatim}


==> FileTex/conclusionstech.tex <==



==> FileTex/stargalaxy.tex <==
One of the most relevant problems in the extraction
of scientifically useful information from wide field astronomical images (both photographic plates and CCD
frames) is the recognition of the objects against a noisy
background and their classification in unresolved (starlike) and resolved (galaxies) sources. In this chapter I present
present two works performed in this area.
